Double Machine Learning based Program Evaluation under Unconfoundedness

This paper reviews, applies and extends recently proposed methods based on Double Machine Learning (DML) with a focus on program evaluation under unconfoundedness. DML based methods leverage flexible prediction models to adjust for confounding variables in the estimation of (i) standard average effects, (ii) different forms of heterogeneous effects, and (iii) optimal treatment assignment rules. An evaluation of multiple programs of the Swiss Active Labour Market Policy illustrates how DML based methods enable a comprehensive program evaluation. Motivated by extreme individualised treatment effect estimates of the DR-learner, we propose the normalised DR-learner (NDR-learner) to address this issue. The NDR-learner acknowledges that individualised effect estimates can be stabilised by an individualised normalisation of inverse probability weights.

==> CATE_distr.tex <==
\begin{figure}[t] % "[t!]" placement specifier just for this example
\caption{Distribution of CATEs} \label{fig:cate-distr}
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\linewidth]{Graphs/RF_CATE/CATE_distr_cens_Job_search.pdf}
\caption{Job search} 
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\linewidth]{Graphs/RF_CATE/CATE_distr_cens_Vocational.pdf}
\caption{Vocational}
\end{subfigure}

\medskip
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\linewidth]{Graphs/RF_CATE/CATE_distr_cens_Computer.pdf}
\caption{Computer} 
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\linewidth]{Graphs/RF_CATE/CATE_distr_cens_Language.pdf}
\caption{Language} 
\end{subfigure}
\subcaption*{\textit{Note:} The dark grey histogram shows the estimated CATE distribution with the five handpicked variables female, age, foreigner, employability and past income. The light grey histogram shows the estimated IATEs and is censored for computer and language programs.}
\end{figure}

==> Tables/Table_OLS_high.tex <==
\begin{table}[htp]
  \centering  \tiny
\begin{threeparttable}[t]
  \caption{Best linear prediction CATEs} 
  \label{tab:cate-ols-high} 
\begin{tabular}{lcccc} 
\toprule
\\[-1.8ex] & \multicolumn{1}{c}{Job search} & \multicolumn{1}{c}{Vocational} & \multicolumn{1}{c}{Computer} & \multicolumn{1}{c}{Language}\\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} \\ 
\midrule
UE female & -2.78$^{*}$ & 12.04$^{**}$ &  5.76 & -1.73 \\ 
   & (1.42) & (4.86) & (4.94) & (3.81) \\ 
  CW age &  0.21 & -1.51 &  1.64$^{*}$ & -1.87$^{**}$ \\ 
   & (0.28) & (0.95) & (0.97) & (0.82) \\ 
  CW female &  0.02 &  0.02 &  0.00 & -0.01 \\ 
   & (0.01) & (0.04) & (0.05) & (0.04) \\ 
  CW tenure & -0.13 & -1.41 &  1.16 & -0.72 \\ 
   & (0.27) & (0.87) & (0.93) & (0.78) \\ 
  CW own unemp experience & -0.01 & -0.05 &  0.04 &  0.01 \\ 
   & (0.04) & (0.15) & (0.15) & (0.12) \\ 
  CW above voc training &  0.04 & -0.65 & -0.29 & -0.21 \\ 
   & (0.27) & (0.88) & (0.93) & (0.76) \\ 
  CW tertiary education &  0.31 & -1.21 &  1.01 &  0.87 \\ 
   & (0.29) & (0.95) & (0.99) & (0.86) \\ 
  CW voc training &  0.27 & -2.52$^{**}$ &  0.82 & -0.52 \\ 
   & (0.36) & (1.21) & (1.22) & (1.05) \\ 
  UE assignment by industry &  0.20 & -0.25 & -1.00 & -0.36 \\ 
   & (0.30) & (0.98) & (1.04) & (0.90) \\ 
  UE assignment by occupation & -0.08 & -0.24 &  0.21 & -0.78 \\ 
   & (0.27) & (0.87) & (0.89) & (0.81) \\ 
  UE assignment by age &  0.29 &  1.43 &  2.05$^{**}$ &  0.89 \\ 
   & (0.27) & (0.89) & (0.92) & (0.78) \\ 
  UE assignment by employability & -0.86 &  0.72 &  0.96 &  1.40 \\ 
   & (0.66) & (2.00) & (2.25) & (1.55) \\ 
  UE assignment by region & -0.03 &  0.48 &  0.81 &  1.14 \\ 
   & (0.48) & (1.47) & (1.52) & (1.02) \\ 
  UE assignment by other & -1.21$^{***}$ &  0.97 &  0.09 & -0.05 \\ 
   & (0.41) & (1.07) & (1.30) & (1.01) \\ 
  UE mother tongue non-Swiss & -0.60 & -0.15 & -2.94 & -1.20 \\ 
   & (0.45) & (1.41) & (1.98) & (1.30) \\ 
  Cantonal unemployment rate &  0.06 &  0.03 & -1.89 & -1.86$^{*}$ \\ 
   & (0.39) & (1.26) & (1.32) & (1.03) \\ 
  \# of unemp. spells in last 2 years &  0.22 & -1.02 &  0.12 & -0.53 \\ 
   & (0.24) & (0.72) & (0.75) & (0.81) \\ 
  \% of months emp. in last 2 years &  0.24$^{**}$ & -1.06$^{**}$ &  0.31 & -0.06 \\ 
   & (0.11) & (0.41) & (0.44) & (0.36) \\ 
  CW cooperative & -1.22$^{**}$ & -1.11 & -0.49 & -0.68 \\ 
   & (0.55) & (1.99) & (2.17) & (1.53) \\ 
  Missing caseworker characteristics &  0.05 & -0.81 &  1.19 & -0.24 \\ 
   & (0.26) & (0.86) & (0.86) & (0.75) \\ 
  Married &  1.07 & -0.59 &  0.56 & -2.30 \\ 
   & (0.70) & (2.47) & (2.49) & (2.03) \\ 
  UE age & -0.63$^{**}$ &  0.74 & -1.28 &  0.03 \\ 
   & (0.29) & (1.00) & (1.08) & (0.84) \\ 
  UE mother tongue in canton's language &  0.03$^{**}$ &  0.10$^{*}$ &  0.04 & -0.04 \\ 
   & (0.02) & (0.05) & (0.06) & (0.04) \\ 
  Cantonal GDP p.c. &  0.19 & -0.72 &  0.02 &  2.16$^{*}$ \\ 
   & (0.46) & (1.54) & (1.88) & (1.17) \\ 
  Past income &  1.53 & -0.77 &  0.02 & 13.95$^{*}$ \\ 
   & (2.09) & (6.30) & (6.87) & (7.33) \\ 
  \# employment spells in last 5 years & -0.23$^{***}$ & -0.55$^{**}$ & -0.48$^{**}$ &  0.12 \\ 
   & (0.08) & (0.26) & (0.22) & (0.20) \\ 
  Medium employability &  0.15 &  3.14 & -1.72 &  0.51 \\ 
   & (0.94) & (3.15) & (3.38) & (2.89) \\ 
  High employability & -0.45 & -1.65 & -2.36$^{*}$ & -1.19 \\ 
   & (0.38) & (1.20) & (1.25) & (1.01) \\ 
  Lives in medium city & -1.06$^{**}$ & -2.70$^{*}$ & -3.53$^{**}$ & -1.43 \\ 
   & (0.53) & (1.56) & (1.76) & (1.52) \\ 
  Lives in big city &  0.28 &  1.22 & -0.76 &  0.03 \\ 
   & (0.40) & (1.33) & (1.52) & (1.19) \\ 
  Qualification semiskilled & -0.23 &  0.40 & -0.49 & -1.45 \\ 
   & (0.38) & (1.36) & (1.32) & (1.06) \\ 
  Qualification no degree &  0.12 &  0.54 & -1.04 &  1.39 \\ 
   & (0.45) & (1.65) & (1.58) & (1.20) \\ 
  Qualification degree & -0.46 & -2.88 & -2.08 &  1.65 \\ 
   & (0.76) & (2.54) & (3.31) & (1.78) \\ 
  Foreigner with B permit &  0.19 &  0.40 & -1.47 &  0.79 \\ 
   & (0.42) & (1.39) & (1.47) & (1.20) \\ 
  Foreigner with C permit &  0.44 &  2.30 &  1.16 & -1.52 \\ 
   & (0.47) & (1.70) & (1.51) & (1.04) \\ 
  Previous job self-employed &  0.33 &  1.66 & -0.95 & -1.55 \\ 
   & (0.38) & (1.23) & (1.44) & (1.07) \\ 
  Previous job manager &  4.38$^{***}$& -4.32 &  3.81 &  7.62$^{***}$\\ 
   & (1.67) & (6.87) & (4.14) & (2.39) \\ 
  Previous job skilled worker & -0.05 & -2.22 & -0.04 &  0.73 \\ 
   & (0.58) & (2.19) & (2.32) & (1.77) \\ 
  Sector missing & -0.57 & -0.04 &  0.63 &  1.03 \\ 
   & (0.37) & (1.26) & (1.32) & (1.03) \\ 
  Previous job in secondary sector &  1.25$^{**}$ & -5.19$^{***}$& -1.70 &  2.49 \\ 
   & (0.56) & (1.79) & (1.64) & (1.58) \\ 
  Previous job in tertiary sector &  0.91 & -0.67 & -0.01 &  2.00 \\ 
   & (0.57) & (1.77) & (1.68) & (1.65) \\ 
  UE female &  0.31 & -2.86$^{*}$ & -1.15 &  2.66$^{*}$ \\ 
   & (0.49) & (1.52) & (1.35) & (1.46) \\ 
  F-statistic & 2.61$^{***}$& 1.59$^{***}$& 1.05 & 1.36$^{*}$ \\
    \bottomrule
    \end{tabular}%
         \begin{tablenotes} \item \textit{Note:} This table shows OLS coefficients and their heteroscedasticity robust standard errors (in parentheses) of regressions run with the pseudo-outcome defined in Section \ref{sec:est-cate} as well as summary statistics about the distribution of the respective best linear predicted CATEs. $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01 \end{tablenotes}  
\end{threeparttable}
\end{table}

==> Tables/Table_optimal_policy_high.tex <==
\singlespacing
\begin{table}[t]
  \centering  \footnotesize
\begin{threeparttable}
  \caption{Description of estimated optimal policies} 
\begin{tabular}{lccccc} 
\toprule
\\[-1.8ex] & \multicolumn{1}{c}{No program} & \multicolumn{1}{c}{Job search} & \multicolumn{1}{c}{Vocational} & \multicolumn{1}{c}{Computer} & \multicolumn{1}{c}{Language}\\ 

\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)}\\ 
\midrule

\multicolumn{6}{l}{\textit{Panel A: Percent allocated to program}} \\
 [0.4em]
 Depth 1 \& 5 variables & 0 & 0 & 56 & 44 & 0 \\ 
 [0.4em]
 Depth 2 \& 5 variables  & 0 & 0 & 57 & 33 & 10 \\ 
 [0.4em]
 Depth 3 \& 5 variables  & 0 & 0 & 32 & 51 & 16 \\ 
  [0.4em]
 Depth 1 \& 16 variables & 0 & 0 & 46 & 0 & 54 \\ 
 [0.4em]
 Depth 2 \& 16 variables & 0 & 0 & 37 & 19 & 46 \\ 
 [0.4em]
 Depth 3 \& 16 variables & 0 & 0 & 42 & 30 & 28 \\ 
 [0.8em]
\multicolumn{6}{l}{\textit{Panel B: Cross-validated difference to APOs}} \\  
[0.4em]
Depth 1 \& 5 variables  & 3.46$^{***}$ & 4.49$^{***}$ & 0.13 & 0.17 & 0.88 \\ 
   & (0.43) & (0.44) & (0.60) & (0.62) & (0.57) \\ 
         [0.4em]
Depth 2 \& 5 variables  &  2.92$^{***}$ &  3.95$^{***}$ & -0.41 & -0.36 &  0.34 \\ 
   & (0.42) & (0.43) & (0.59) & (0.61) & (0.56) \\ 
         [0.4em]
 Depth 3 \& 5 variables &  2.97$^{***}$ &  4.00$^{***}$ & -0.36 & -0.32 &  0.39 \\ 
        & (0.42) & (0.43) & (0.50) & (0.47) & (0.47) \\ 
 [0.4em]
Depth 1 \& 16 variables & 3.60$^{***}$ & 4.63$^{***}$ & 0.27 & 0.32 & 1.02$^{**}$ \\ 
   & (0.42) & (0.43) & (0.44) & (0.58) & (0.41) \\ 
         [0.4em]
Depth 2 \& 16 variables  & 3.70$^{***}$ & 4.73$^{***}$ & 0.37 & 0.41 & 1.12$^{***}$ \\ 
   & (0.41) & (0.43) & (0.48) & (0.52) & (0.43) \\ 
         [0.4em]
Depth 3 \& 16 variables & 3.58$^{***}$ & 4.61$^{***}$ & 0.25 & 0.30 & 1.01$^{**}$ \\ 
   & (0.44) & (0.45) & (0.47) & (0.49) & (0.49) \\

    \bottomrule
    \end{tabular}%
         \begin{tablenotes} \item \textit{Note:} Panel A show the percentage of individuals that are assigned to a specific program by the trees of different depth. Panel B show a t-test of the difference of the cross-validated policy (standard errors in parentheses) and the APOs of the programs. $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01 \end{tablenotes}  
\end{threeparttable}
\end{table}
\doublespacing
